Efficient Scene Appearance Aggregation for Level-of-Detail Rendering

Creating an appearance-preserving level-of-detail (LoD) representation for arbitrary 3D scenes is a challenging problem. The appearance of a scene is an intricate combination of both geometry and material models, and is further complicated by correlation due to the spatial configuration of scene elements. We present a novel volumetric representation for the aggregated appearance of complex scenes and an efficient pipeline for LoD generation and rendering. The core of our representation is the Aggregated Bidirectional Scattering Distribution Function (ABSDF) that summarizes the far-field appearance of all surfaces inside a voxel. We propose a closed-form factorization of the ABSDF that accounts for spatially varying and orientation-varying material parameters. We tackle the challenge of capturing the correlation existing locally within a voxel and globally across different parts of the scene. Our method faithfully reproduces appearance and achieves higher quality than existing scene filtering methods while being inherently efficient to render. The memory footprint and rendering cost of our representation are independent of the original scene complexity.

==> old_correlation.tex <==
\section{Correlation-aware Visibility and Coverage} \label{sec:correlation}
A core challenge for all scene aggregation methods is the correlation existing between the scene geometry. This is because these methods are motivated to
simplify the original scene, which usually means discretizing the scene at a finite resolution, e.g., voxelization. As mentioned in \S \ref{subsec:measure_pixel},
Each discrete element is then represented
by a simple primitive, e.g., a voxel in the simplest case. Compared to the original representation, two pieces of important information are lost with this
na\"ive simplified representation. We first demonstrate how the na\"ive discretization loses track of
the geometrical relationship between voxels and how the AIV helps preserve this correlation by recording the \emph{global} visibility with origins inside a voxel.
As the discretization processes each voxel individually, the best assumption it can make without further information is that the surfaces are independently
distributed in each voxel.
Consider a pair of subsets of the scene $A_1$, $A_2$ and their corresponding voxels $B_1$, $B_2$. Given a ray that hits $A_1$,
its true conditional probability to hit $A_2$ can be drastically different from that when we assume surfaces are independently distributed in $B_1$ and $B_2$.
This is best explained through a set of examples in 2D flatland. In the \emph{inter-voxel occlusion} example in Fig.~\ref{fig:intervoxel_correlation},
we uniformly cast rays to three aligned voxels $B_i$, each containing a
piece of (1D) geometry $A_i$ with color $c_i$. The perceived color is obtained by averaging the color on the hit points of all rays. In
Fig.~\ref{fig:intervoxel_correlation}~(a), the observed
color is $0.5c_1 + 0.5c_3$ as $A_2$ is completed occluded by $A_1$. In other words, a ray must hit $A_2$ if it hits $A_1$. In Fig.~\ref{fig:intervoxel_correlation}~(b), $A_2$ is moved so that
it is no longer occluded while $A_3$ is occluded. The observed color is $0.5c_1 + 0.5c_2$. However, the na\"ive assumption (Fig.~\ref{fig:intervoxel_correlation}~(c))
leads to an incorrect result of $0.5c_1 + 0.25c_2 + 0.25c_3$ that matches neither configuration because it does not account for the correlation between voxels.
Our method correctly resolves this ambiguity because the AIV encodes global visibility (Fig.~\ref{fig:intervoxel_correlation}~(d)).

While the AIV reconstruts the inter-voxel correlation, it does not help resolve how geometry is distributed locally inside each voxel.
This information is again lost during the discretization and the best assumption we can
make is that the surfaces are uniformly distributed in the voxel, akin to how particles are distributed in a volume. However, the uniform assumption is poor
in practice especially since many 3D assets comprise large pieces of flat surfaces. Typically, this is visible for a voxel around the silhouette as shown in
Fig.~\ref{fig:silhouette}, where only a half of the voxel is occupied, while the other half is completely unoccupied. After discretization, however, this correlation
is lost that results in a uniformly transparent block.

\begin{figure}[tb]
    \centering
    \begin{tabular}{cc}
        \includegraphics[width=1.5in]{imgs/illustration/intervoxel_correlation_1.png}
        &
        \includegraphics[width=1.5in]{imgs/illustration/intervoxel_correlation_2.png} \\
        (a) & (b) \\
        \includegraphics[width=1.5in]{imgs/illustration/intervoxel_correlation_3.png}
        &
        \includegraphics[width=1.5in]{imgs/illustration/intervoxel_correlation_4.png} \\
        (c) & (d)
    \end{tabular}
    \caption{\label{fig:intervoxel_correlation}
        (a) and (b): Tracing rays against correlated geometry produces different results depending on different configurations. (c): Ignoring such correlation
        leads to incorrect result. (d): The global visibility in ABSDF (Eq.~\ref{eq:absdf_def}) helps recover the correlation in (b) by excluding the invisible
        contribution from $A_2$.
    }
\end{figure}

The next \emph{double-counting} example presents a trickier issue with more objectionable artifacts. In Fig.~\ref{fig:double-counting},
a connected piece of geometry $A$ is discretized into two diagonally neighboring voxels $B_1$ and $B_2$, each containing a part of $A$, $A_1$ and $A_2$. When casting rays
from a non-axis-aligned direction, some rays will overlap both voxels, resulting in double counting the contribution from both voxels. In this case, the fact that
the ABSDF encodes global visibility is irrelevant because there is no occlusion between any pair of points on $A$. Again, the fundamental reason for this issue
is the correlation between voxel: with the original geometry, whenever a ray hits $A_1$, it will never hit $A_2$. This information is lost after
the discretization and there is no such property between $B_1$ and $B_2$ (except from the axis-aligned directions).

It is important to realize that the correlation is defined by the very geometry itself.
Theoretically, one trivial solution to handle correlation is to increase the resolution of the discretization to approximate arbitrary types of geometry.
It is not hard to see that the error in all
three examples discussed previously vanishes as the resolution approaches infinity. However, this implies that we may only expect reasonably correct results
when the discretization resolution is much finer than the pixel footprint, which is impractical. Importantly, we emphasize that following the Nyquist-Shannon sampling
theorem and setting the resolution at half the size of pixel footprint is not enough because the scene aggregation problem is more than a pure image space signal
reconstruction problem. One should also pay attention to the spatial frequency of the scene geometry when sampling it with finite resolution.
Unfortunately, it is often unbounded because the geometry is often modeled by polygon-based boundary representation.
Common approaches that introduce further subdivision within a single voxel, such as using a coverage mask, are essentially no different than simply increasing the
resolution. Alternatively, we can improve the primitive $B$ for a scene subset $A$ such that the results converge faster as the
resolution increases. This can be particularly effective while only incurring a small extra cost, as we demonstrate in the following.

\begin{figure}[h]
    \centering
    \includegraphics[height=1in]{imgs/illustration/silhouette_1.png} \\
    \caption{\label{fig:silhouette}
        In this example, a voxel around the silhouette of an object is half occupied. However, the discretization does not preserve this correlation and produces a
        blocky look.
    }
\end{figure}

\begin{figure}[tb]
	\newlength{\heightDoubleCounting}
	\setlength{\heightDoubleCounting}{0.8in}
    \addtolength{\tabcolsep}{-7pt}
    \renewcommand{\arraystretch}{0.5}
    \centering
    \begin{tabular}{ccc}
        \includegraphics[height=\heightDoubleCounting]{imgs/illustration/double_counting_1.png}
        &
        \includegraphics[height=\heightDoubleCounting]{imgs/illustration/double_counting_2.png}
        &
        \includegraphics[height=\heightDoubleCounting]{imgs/illustration/double_counting_3.png}
        \\
        (a) & (b) & (c)
    \end{tabular}
    \caption{\label{fig:double-counting}
        (a): It is only possible to hit once when tracing against the connected piece of geometry. (b): However, the correlation is not preserved with na\"ive
        discretization. (c): The truncated ellipsoid primitive greatly improves the situation by better adapting to the geometry.
    }
\end{figure}

\subsection{Truncated Ellipsoid Primitive} \label{subsec:ellip}
We propose to fit a bounding ellipsoid for the geometry $A$ within each voxel and define the new primitive $B$ as the intersection of the voxel and the
ellipsoid. The new truncated ellipsoid primitive is still a bounding volume of $A$. The new primitive is much more effective at adapting to the shape of $A$:
when $A$ comprises a flat surface or a fiber-like thin structure, $B$ now provides a much tighter fit and greatly reduces both the silhouette error and the
double-counting error; when $A$ comprises unstructured geometry that fills the voxel, $B$ falls back to a box shape. The truncated ellipsoid primitive
provides a good tradeoff in practice as it is easy to fit and compact to store. See \S \ref{subsec:precompute} for details. Note that we
never need to explicitly store the box-ellipsoid intersection; it is sufficient to store the separate shapes and calculate the properties of the intersection
on-the-fly. We validate the effectiveness of this strategy in Fig.~\ref{fig:validate_ellipsoid}. In particular, the na\"ive primitive produces the
checkerboard-like pattern for the red plane example. This is not Monte Carlo noise, but the manifestation of the double-counting artifact.
This is also not due to ``insufficient'' voxel resolution because the voxel size is already small than pixel footprint. In contrast, our method not only
produces a tighter silhouette but also does not suffer from the artifact.

We now re-examine Eq. \ref{eq:measure_eq_farfield} as the choice of $B$ affects the calculation of several terms in it, namely $|P^+_k|$ and
$\hat{C}_{A_k}(\omega_\mathrm{f}; P^+_k)$. $|P^+_k|$ is calculated by either ray casting or rasterization and the ray intersection test for the truncated ellipsoid
primitive is only slightly more costly than the ray-voxel test. The calculation of the directional primitive coverage $\hat{C}_{A_k}(\omega_\mathrm{f}; P^+_k)$ depends on how
$A_k$ ($B_k$) partially overlaps a particular pixel footprint $P^+_k$. Under the far-field assumption, however, it is reasonable to drop the dependency on $P^+_k$:
\begin{equation} \label{eq:primitive_coverage}
    \hat{C}_{A_k}(\omega_\mathrm{f}; P^+_k) \approx \hat{C}_{A_k}(\omega_\mathrm{f}) = \frac{|A_k(\omega_\mathrm{f})|}{|B_k(\omega_\mathrm{f})|},
\end{equation}
where $B_k(\omega_\mathrm{f})$ is the parallel-projection of $B_k$ and $B_k(\omega_\mathrm{f})$ is the projected area. Note that there is no need to explicitly
calculate $|A_k(\omega_\mathrm{f})|$ since it cancels out with the terms in Eq. \ref{eq:absdf_distrib}. This leaves us to the problem of calculating
the projected area of the $|B_k(\omega_\mathrm{f})|$. Unlike the na\"ive box primitive whose projected area is trivial to calculate, there is no closed-form
solution to calculate the projected area of the intersection of a cube and an ellipsoid to the best of our knowledge. We resort to an efficient Monte Carlo estimator
detailed in the supplemental document.

\begin{figure}[h]
	\newlength{\lenValidateEllipsoid}
	\setlength{\lenValidateEllipsoid}{0.8in}
    \addtolength{\tabcolsep}{-4pt}
    \renewcommand{\arraystretch}{0.5}
    \centering
    \begin{tabular}{ccc}
        \frame{\includegraphics[height=\lenValidateEllipsoid]{imgs/validate_ellipsoid_redplane/pt_img32_redplane.png}}
        &
        \frame{\includegraphics[height=\lenValidateEllipsoid]{imgs/validate_ellipsoid_redplane/naive_lod32_redplane.png}}
        &
        \frame{\includegraphics[height=\lenValidateEllipsoid]{imgs/validate_ellipsoid_redplane/ellipsoid_lod32_redplane.png}}
        \\
		\multicolumn{1}{r}{\frame{\begin{overpic}[height=\lenValidateEllipsoid,unit=1mm]{imgs/colorbar.png}
			\put(-20, 91){\normalsize 0.1}
			\put(-20, 1){\normalsize 0.0}
		\end{overpic}}}
        &
        \frame{\includegraphics[height=\lenValidateEllipsoid]{imgs/validate_ellipsoid_redplane/diff_naive_lod32_redplane.png}}
        &
        \frame{\includegraphics[height=\lenValidateEllipsoid]{imgs/validate_ellipsoid_redplane/diff_ellipsoid_lod32_redplane.png}}
        \\
        (a) PT Ref. & (b) Na\"ive $32^3$ & (c) Ours $32^3$
    \end{tabular}
    \caption{\label{fig:validate_ellipsoid}
        Compared to the reference, LoD with na\"ive primitive results in bloated silhouette and worse, structured artifacts on the red plane.
        With the help of the truncated ellipsoid primitive, our method produces a tighter silhouette and more importantly, artifact free results.
        We encourage readers to zoom in to better identify the checkerboard-like artifact.
    }
\end{figure}


==> old_factoring.tex <==
\section{Factoring Aggregated Appearance} \label{sec:factoring}
According to Eq. \ref{eq:absdf_def}, an ABSDF is defined by integrating the product of base material, foreshortening factors, and bidirectional visibility over
the underlying surfaces. This is challenging, as in general, no closed-form solution exists. However, we would also like to avoid stochastic evaluation or
numerical integration which would greatly greatly increase the rendering cost and undermine the purpose of scene aggregation. To achieve closed-form evaluation and
importance sampling, we factor the ABSDF with the following steps.

\emph{Separate Visibility}.
We perform a splitting approximation that separate the integration of the bidirectional visibility from the rest:
\begin{align} \label{eq:split_vis}
\begin{split}
        \hat{f}(\omega_i, \omega_o) \approx
        \frac{1}{|A|_{\omega_o}} &\int_A f(x,\omega_i, \omega_o) \langle n_x\cdot\omega_i \rangle \langle n_x\cdot\omega_o \rangle \,\D{x} \\
        \frac{1}{|A|} &\int_A V(x, \omega_i) V(x, \omega_o)  \,\D{x}. \\
\end{split}
\end{align}
The aggregated bidirectional visibility is still a 4D function that requires infeasible storage. We further
separates the integration of each direction:
\begin{align} \label{eq:split_split_vis}
\begin{split}
    \frac{1}{|A|}\int_A V(x, \omega_i) V(x, \omega_o)  \,\D{x} \approx
    &\frac{1}{|A|} \int_A V(x, \omega_i) \,\D{x} \frac{1}{|A|}\int_A V(x, \omega_o)  \,\D{x}  \\
    = &\hat{V}(\omega_i) \hat{V}(\omega_o).
\end{split}
\end{align}
The \emph{aggregated interior visibility} (AIV) $\hat{V}(\omega)$ is now a 2D function, which we represent by Haar wavelet coefficients. We discuss further
strategies to compress its storage in \S \ref{subsec:compression}.

\emph{Base material}.
The ABSDF is dependent on the underlying surface base materials. For the widest applicability, it
is desirable to support material models used by existing assets. Therefore, we target the Disney Principled BRDF \cite{burley2012physically}, which is one of the most
commonly used models in production and capable of recreating a wide range of appearance. The Disney BRDF is a sophisticated model consisting of multiple lobes.
We preserve its core feature but make three simplifications to the original model:
\begin{enumerate}
    \item For diffuse reflection, we use the simpler Lambertian model instead of the original empirical model with retro-reflection. The difference is
          insignificant when viewing from far field.
    \item We omit the optional sheen and clearcoat lobes.
    \item We assume surfaces are double-sided. This is only for technical convenience.
\end{enumerate}

The modified model can be written as
\begin{align}
\begin{split}
    f_{\text{disney}}(\omega_i, \omega_o) &= f_{s}(\omega_i, \omega_o) + f_d(\omega_i, \omega_o), \\
    f_{s}(\omega_i, \omega_o) &= \frac{ D(\omega_h; \alpha) G(\omega_i, \omega_o; \alpha) }{ 4 | n, \omega_o | | n, \omega_i | }
    \Big( \beta^m F(\omega_h, \omega_o;\beta^c) + \\
    & \quad (1 - \beta^m) F(\omega_h, \omega_o;\beta^s) \Big), \\
    f_{d}(\omega_i,  \omega_o) &= \frac{(1 - \beta^m) \beta^c}{\pi}, \\
\end{split}
\end{align}
where $f_{s}(\omega_i, \omega_o)$ is the specular component that consists of both metallic and dielectric Fresnel reflection,
$f_d(\omega_i, \omega_o)$ is the diffuse component,
$D(\omega_h)$ is the Trowbridge-Reitz (GGX) distribution as the microfacet distribution,
$F(\omega_h)$ is the (Schlick) Fresnel equation, and $G(\omega_i, \omega_o)$ is the shadowing-masking function. The model is controlled by a set of parameters
$\beta \coloneqq (\alpha, \beta^c, \beta^m, \beta^s) = $ (roughness, basecolor, metallic, specular intensity), which can all be spatially-varying.

\emph{The distribution form of ABSDF}.
With the visibility terms separated, we convert the ABSDF into a convolution between the base material and the joint distribution of material parameters.
Similar operations have been employed in normal map and displacement map filtering techniques~\cite{han2007frequency,olano2010lean,dupuy2013linear}, but they
usually only consider the distribution of surface normals (NDF). Our formulation can be seen as a generalization that incorporates all spatially-varying parameters.
Let $\gamma_x\coloneqq (n_x, \beta_x)$ be a vector consisting of surface normal and all material parameters at $x$. It can also be interpreted
as a value of a random vector $Y$ with joint PDF $p_{Y}(\gamma)$. We can rewrite the ABSDF (no visibility) as follows:
\begin{align} \label{eq:absdf_distrib}
\begin{split}
    \hat{f}_{\mathrm{novis}}(\omega_i, \omega_o)
    &=\frac{1}{|A|_{\omega_o}} \int_A f(\omega_i,\omega_o; \beta_x) \langle n_x\cdot\omega_i \rangle \langle n_x\cdot\omega_o \rangle\,\D{x} \\
    &=\frac{|A|}{|A|_{\omega_o}} \int_{\Gamma} f(\omega_i,\omega_o; \beta) \langle n\cdot\omega_i \rangle \langle n\cdot\omega_o \rangle p_{Y}(\gamma) \,\D{\gamma},
\end{split}
\end{align}
where $\Gamma$ is the product space of all parameters. We now focus on factoring of each component.

\subsection{Factoring The Specular Component} \label{subsec:factoring_specular}
We substitute $f_s(\omega_i, \omega_o)$ into the integral of Eq. \ref{eq:absdf_distrib} and expand it as
\begin{align} \label{eq:factor_specular}
\begin{split}
    \int_{\Gamma} &f_s(\omega_i,\omega_o; \beta) \langle n\cdot\omega_i \rangle \langle n\cdot\omega_o \rangle p_{Y}(\gamma) \,\D{\gamma} = \\
    &\frac{1}{4} \Big[ (1-\mathcal{F}_c) \, \boxed{\int_{\Gamma} \mathcal{R} \mathcal{D} p_{Y}(\gamma) \,\D{\gamma}} + \mathcal{F}_c \int_{\Gamma} \mathcal{D} p_{Y}(\gamma) \,\D{\gamma} \Big], \\
    &\mathcal{F}_c = 1 - \cos^5(|\omega_h \cdot \omega_o|), \\
    &\mathcal{R} = \beta^m \beta^c + (1-\beta^m)\beta^s, \\
    &\mathcal{D} = D(\omega_h; n, \alpha) G(\omega_i, \omega_o; n, \alpha) \chi^+(n \cdot \omega_o) \chi^+(n \cdot \omega_i), \\
\end{split}
\end{align}
where $\mathcal{F}_c$ is the Schlick factor and $\chi^+(\cdot)$ is the Heaviside function. Note that $\chi^+(n \cdot \omega_o)$ and $\chi^+(n \cdot \omega_i)$
appear due to the clamped dot products in Eq. \ref{eq:absdf_distrib}. We split the highlighted integral in Eq. \ref{eq:factor_specular} by assuming
$p_{Y}(\gamma) \approx p_{Y_1}(\beta^c, \beta^m, \beta^s) p_{Y_2}(n, \alpha)$:
\begin{equation} \label{eq:specular_orient_split}
    \int_{\Gamma} \mathcal{R} \mathcal{D} p_{Y}(\gamma) \,\D{\gamma} \approx
    \int_{\Gamma_1} \mathcal{R} p_{Y_1}(\gamma) \,\D{\gamma} \,\boxed{\int_{\Gamma_2} \mathcal{D} p_{Y_2}(\gamma)} \,\D{\gamma},
\end{equation}

where $\Gamma_1$ and $\Gamma_2$ is the product space of $(\beta^c, \beta^m, \beta^s)$ and $(n, \alpha)$, respectively.
Doing so implies $\beta^c$, $\beta^m$, and $\beta^s$ are orientation-independent. We extend our formulation to handle orientation-varying parameters in
\S \ref{subsec:orient}. After the splitting, the left integral can be simply represented by the means and second-order moments of the parameters
\begin{equation}
    \int_{\Gamma_1} \mathcal{R} p_{Y_1}(\gamma) \,\D{\gamma} = \mathbb{E}[\beta^m \beta^c] + \mathbb{E}[\beta^s] - \mathbb{E}[\beta^m \beta^s].
\end{equation}
For the highlighted right integral, we propose a closed-form solution with several small, scene-independent precomputed tables. The solution can be broken down to several parts:

\emph{Handling normal variation.} Similar to normal map filtering and specular shading antialiasing techniques~\cite{olano2010lean, kaplanyan2016filtering},
the variation of surface normals can be treated by convolving the surface NDF $p_N(n)$ function by the microfacet distribution $D(\omega_h)$.
This results in a convolved distribution $D_\mathrm{conv}(\omega_h)$ that is smoother. We use the SGGX distribution~\cite{heitz2015sggx} to represent the surface NDF in
$A$: $p_N(n) = D_{\mathrm{sggx}}(n)$ and utilize the fact that an SGGX is equivalent to a double-sided GGX. Given an SGGX matrix $S$ with eigenbasis $(\omega_1, \omega_2, \omega_3)$
and projected area $\sigma(\omega_1) \leq \sigma(\omega_2) \leq \sigma(\omega_3)$, we can always scale the entire matrix by $1/\sigma^2(\omega_3)$.
The result is still a valid SGGX matrix:
\begin{equation}
    S' = \frac{S}{\sigma^2(\omega_3)} =
    (\omega_1, \omega_2, \omega_3)
    \begingroup %
    \setlength\arraycolsep{1pt}
    \begin{pmatrix}
    \frac{\sigma^2(\omega_1)}{\sigma^2(\omega_3)} & 0 & 0\\
    0 & \frac{\sigma^2(\omega_2)}{\sigma^2(\omega_3)} & 0\\
    0 & 0 & 1
    \end{pmatrix}
    \endgroup
    (\omega_1, \omega_2, \omega_3)^T,
\end{equation}
It is shown by Heitz et al.~\shortcite{heitz2015sggx} that $S'$ is a double-sided GGX with roughness $\alpha_x = \sigma(\omega_1) / \sigma(\omega_3)$,
$\alpha_y = \sigma(\omega_1) / \sigma(\omega_3)$, and tangent frame $R = (\omega_1, \omega_2, \omega_3)$.
Since we assume surfaces are double-sided, the microfacet distribution $D(\omega_h)$ also becomes an
(isotropic) SGGX. Thus, the problem is reduced to the convolution between an anisotropic SGGX and an isotropic SGGX. We propose to represent this convolution
by a new anisotropic SGGX with the same eigenvectors as the original SGGX:
\begin{align} \label{eq:sggx_conv}
\begin{split}
    D_\mathrm{conv}(\omega_h) &= \int_{\mathbb{S}^2} D(\omega_h; \omega', \alpha) p_N(\omega') \, \D{\omega'} \\
    &=\int_{\mathbb{S}^2} D_{\mathrm{sggx}}(\omega_h; \omega', \alpha) D_{\mathrm{sggx}}(\omega'; R, \alpha_x, \alpha_y) \, \D{\omega'} \\
    &\approx D_{\mathrm{sggx}}(\omega_h; R, \alpha_x + \Delta \alpha_x, \alpha_y + \Delta \alpha_y),
\end{split}
\end{align}
where $\Delta \alpha_x$ and $\Delta \alpha_y$ are the additional roughness gained due to the convolution.
This is inspired by Xu et al.~\shortcite{xu2013anisotropic}, where a similar approximation is made for anisotropic Spherical Gaussian that turns out to be
very accurate. While Xu et al. seeks an symbolic approximation, we simply perform a nonlinear least-square fit to find the best mapping
$(\Delta \alpha_x, \Delta \alpha_y) = M_1(\alpha_x, \alpha_y, \alpha)$ and store it as a small 3D table. 
Note that the original SGGX distribution is unnormalized, but we prefer normalized distributions in Eq. \ref{eq:sggx_conv}. Fortunately the norm of GGX is a
very smooth function ranging within $[1,2]$ and easy to precompute as another small 2D table
$\int_{\mathbb{H}^2} D_{\mathrm{GGX}}(\omega; \alpha_x, \alpha_y)\, \D{\omega} = M_2(\alpha_x, \alpha_y)$, and the corresponding SGGX distribution has twice the norm.

In cases when the surface NDF is multi-modal, we use an SGGX mixture with a small number of components, namely
\begin{equation} \label{eq:multi_lobe_ndf}
    p_N(n) = \sum_{i=1}^k w_i D_{\mathrm{sggx}}(n; R^i, \alpha_x^i, \alpha_y^i),
\end{equation}
where each lobe is processed separately as described by Eq.~\ref{eq:sggx_conv}. See Fig.~\ref{fig:absdf_plot} for an example where a mixture model is useful.
We describe the fitting process for the mixture model in \S~\ref{subsec:precompute}.

\emph{Handling roughness variation.}
The roughness $\alpha$ can also be varying on the surfaces of $A$, which means that the microfacet distribution can no longer be represented by one GGX lobe.
Let $\mathcal{A}$ be the underlying random variable for the roughness and
$p_{\mathcal{A}}(\alpha)$ be its marginal density function. The aggregated microfacet distribution is the expectation of the microfacet
distribution
\begin{equation} \label{eq:rough_var}
\mathbb{E}_{\mathcal{A}}[D](\omega) = \int_{[0,1]}  D(\omega; \alpha) p_{\mathcal{A}}(\alpha) \, \D{\alpha}.
\end{equation}
We should represent $p_{\mathcal{A}}(\alpha)$ by a parametric distribution while acknowledging that $\alpha$ is bounded in [0,1]. A Gaussian distribution is thus
not a valid choice. Instead, we use a Beta distribution $\mathcal{B}(\alpha; a, b)$ which has the correct support, is reasonably
expressive, and is easy to estimate.
Eq. \ref{eq:rough_var} can be interpreted as the weighted average of infinite GGX lobes with different possible $\alpha$. Since there is no closed-form
solution for it, we further propose to approximate $\mathbb{E}_{\mathcal{A}}[D](\omega)$ by a weighted average of 2 lobes:
\begin{equation}
    \mathbb{E}_{\mathcal{A}}[D](\omega) \approx m_1D(\omega; \alpha_1) + m_2D(\omega; \alpha_2),
\end{equation}
where $m_1+m_2=1$.
The approximation can be extended to use arbitrary $k$ lobes, but we find $k=2$ provide a good balance between cost and accuracy. Again, we perform a nonlinear
lease square fit to find the best mapping $(m_1, \alpha_1, \alpha_2) = M_3(a, b)$ given the shape parameters of the Beta distribution and store it as a 
small 2D table. For the $i$-th NDF component, the post convolution distribution now becomes
\begin{equation} \label{eq:sggx_conv_2}
        D_\mathrm{conv}^i(\omega_h) =
        \sum_{j} m_j D_{\mathrm{sggx}}(\omega; R^i, \alpha_x^i + \Delta \alpha_x^j, \alpha_y^i + \Delta \alpha_y^j).
\end{equation}

\emph{Restricting angular integration domain.}
So far, we have ignored the Heaviside (step) function terms $\chi^+(n \cdot \omega_i)$ and $\chi^+(n \cdot \omega_o)$ in $\mathcal{D}$. Alternatively, when integrating
$\mathcal{D}p_{Y}(\gamma)$, the angular domain should not be the full sphere $\mathbb{S}^2$, but only a subset
$\mathcal{X} \coloneqq \{ \omega \in \mathbb{S}^2 | (n \cdot \omega_i)(n \cdot \omega_o) > 0 \}$. Intuitively speaking, the restricted domain avoids the
incorrect contribution when $\omega_i$ and $\omega_o$ are from different sides of the surface Otherwise, the ABSDF will suffer from leaking.
This complicates the problem because Eq. \ref{eq:sggx_conv} is not exactly a spherical convolution when the integration domain is $\mathcal{X}$. To preserve the
efficient convolution-based solution while addressing the potential leaking, we apply the following approximation:
\begin{align} \label{eq:angular_domain}
\begin{split}
        \int_{\mathcal{X}} &D_{\mathrm{sggx}}(\omega; \omega', \alpha) D_{\mathrm{sggx}}(\omega'; R^i, \alpha_x^i, \alpha_y^i) \, \D{\omega'} \approx \\
        &D^i_\mathrm{conv}(\omega_h) \int_{\mathcal{X}} D_{\mathrm{sggx}}(\omega; R^i, \alpha_x^i, \alpha_y^i) \,\D{\omega}.
\end{split}
\end{align}
In other words, we scale Eq. \ref{eq:sggx_conv} uniformly by the probability of $\omega$ lying inside $\mathcal{X}$ based on the preconvolved surface normal
distribution. We notice that $\mathcal{X}$ is formed by a (double-sided) intersection of two hemispheres and each piece of the intersection is a spherical
digon. We utilize the Spherical Pivot Transform to achieve closed-form solution for this kind of spherical integration~\cite{dupuy2017spherical}. We fit the pivot
transform to another small 2D table $r_p = M_4(\alpha_x, \alpha_y)$.

Finally, we utilize the fact that the microfacet shadowing-masking term $G(\omega_i, \omega_o; \alpha)$ is very smooth 
~\cite{AshikminPS00,wang2009all,kaplanyan2016filtering}. Therefore, we simply multiply it to each lobe post convolution. Combining this with 
Eq.~\ref{eq:sggx_conv}. \ref{eq:multi_lobe_ndf}, \ref{eq:sggx_conv_2}, and \ref{eq:angular_domain}, we arrive at:
\begin{align} \label{eq:factor_spec_final}
    \begin{split}
    \int_{\Gamma_2} &\mathcal{D} p_{Y_2}(\gamma) \,\D{\gamma} \approx \sum_{i=1}^k w_i S^i(\omega_i, \omega_o) \sum_{j=1}^2 m_{ij} D^{ij}_{\mathrm{sggx}}(\omega_h) G^{ij}(\omega_i, \omega_o) \\
    & S^i(\omega_i, \omega_o) = \int_{\mathcal{X}} D_{\mathrm{sggx}}(\omega; R^i, \alpha_x^i, \alpha_y^i) \,\D{\omega} \\
    & D^{ij}_{\mathrm{sggx}}(\omega_h) = D_{\mathrm{sggx}}(\omega_h; R^i, \alpha_x^i + \Delta \alpha_x^j, \alpha_y^i + \Delta \alpha_y^j) \\
    & G^{ij}(\omega_i, \omega_o) = G(\omega_i, \omega_o, R^i, \alpha_x^i + \Delta \alpha_x^j, \alpha_y^i + \Delta \alpha_y^j),
    \end{split}
\end{align}
which can be evaluated in closed form given the surface NDF $p_N(n)$ and the first two moments of roughness $\alpha$.

\subsection{Factoring The Diffuse Component} \label{subsec:factoring_diffuse}
Next, we substitute $f_d(\omega_i, \omega_o)$ into the integral of Eq. \ref{eq:absdf_distrib} and perform a split similar to Eq.
\ref{eq:specular_orient_split}:
\begin{align} \label{eq:diffuse_orient_split}
\begin{split}
&\int_{\Gamma} f_d(\omega_i,\omega_o; \beta) \langle n\cdot\omega_i \rangle \langle n\cdot\omega_o \rangle p_{Y}(\gamma) \,\D{\gamma} \approx \\
&\int_{\Gamma_1} \frac{(1 - \beta^m) \beta^c}{\pi} p_{Y_1}(\gamma) \,\D{\gamma}
\int_{\mathbb{S}^2} \langle n\cdot\omega_i \rangle \langle n\cdot\omega_o \rangle p_N(n) \,\D{n},
\end{split}
\end{align}
where $p_N(n)$ is the surface NDF (roughness $\alpha$ is irrelevant). Again, the left integral can be immediately simplified to the
means and second-order moments of the parameters
\begin{equation}
    \int_{\Gamma_1} \frac{(1 - \beta^m) \beta^c}{\pi} p_{Y_1}(\gamma) \,\D{\gamma} = \frac{1}{\pi} (\mathbb{E}[\beta^c] - \mathbb{E}[\beta^m\beta^c]).
\end{equation}
For the right integral, we follow Wang et al.~\shortcite{wang2009all} and fit the clamped dot product function by 2 Spherical Gaussian (SG) lobes
$\langle n\cdot\omega \rangle \approx a_1\mathrm{SG}(\omega; n, \kappa_1 ) + a_2\mathrm{SG}(\omega; n, \kappa_2)$, where $a_i$ and $\kappa_i$ are the respective
amplitudes and concentration parameters. Because SGs are closed under multiplication with closed-form expression~\cite{wang2009all}, we can expand the right
integral of Eq. \ref{eq:diffuse_orient_split} as
\begin{align} \label{eq:diffuse_sg}
\begin{split}
    \int_{\mathbb{S}^2} &\langle n\cdot\omega_i \rangle \langle n\cdot\omega_o \rangle p_{N}(n) \,\D{n} \approx\\
    \int_{\mathbb{S}^2} &(a_{11}\mathrm{SG}_{11} + a_{12}\mathrm{SG}_{12} + a_{22}\mathrm{SG}_{22}) D_{\mathrm{sggx}}(n;R, \alpha_x, \alpha_y) \,\D{n}, \\
    &\mathrm{SG}_{ij} = \mathrm{SG}(n; \mu_{ij}, \kappa_{ij}).
\end{split}
\end{align}
We refer readers to Wang et.al~\shortcite{wang2009all} for the full expressions of $a_{ij}$, $\mu_{ij}$, and $\kappa_{ij}$. 
The problem is then reduced to the convolution between a $\mathrm{SG}$ and an SGGX. We employ a
similar strategy to that in \S \ref{subsec:factoring_specular} by representing the result by a new anisotropic SGGX with the same eigenvectors as the original SGGX.
This comes with a new table $(\Delta \alpha_x, \Delta \alpha_y) = M_5(\alpha_x, \alpha_y, \kappa)$. Eq.~\ref{eq:diffuse_sg} then can be evaluated in closed form 
given the surface NDF $p_N(n)$.

The method proposed in \S \ref{subsec:factoring_specular} and \S \ref{subsec:factoring_diffuse} requires a total of 5 precomputed tables. We note that these
are \emph{scene-independent} and only requires precomputation once. Furthermore, most of the mappings are smooth and thus only require a fairly small resolution. The total
storage for the tables are less than 5MB in practice.

In Fig.~\ref{fig:absdf_plot}, we compare our factored ABSDF to the ground truth. The \emph{Helmet} example presents a particularly challenging case with near-specular
anisotropic highlight, which we are able to reconstruct well. For the \emph{Palm} example, we are able to capture the dual-modal shape reasonably well thanks to
our multi-lobe surface NDF representation.

\begin{figure}[t]
	\newlength{\lenABSDFPlot}
	\setlength{\lenABSDFPlot}{1in}
    \addtolength{\tabcolsep}{-4pt}
    \renewcommand{\arraystretch}{0.5}
    \centering
    \begin{tabular}{cccc}
        \raisebox{25pt}{\rotatebox{90}{\emph{Helmet}}}
        &
        \frame{\includegraphics[height=\lenABSDFPlot]{imgs/validate_absdf_plot/helmet_absdf_plot_setup.pdf}}
        &
        \frame{\includegraphics[height=\lenABSDFPlot]{imgs/validate_absdf_plot/helmet_gt_ev+6.png}}
        &
        \frame{\includegraphics[height=\lenABSDFPlot]{imgs/validate_absdf_plot/helmet_ours_ev+6.png}}
        \\
        \raisebox{25pt}{\rotatebox{90}{\emph{Palm}}}
        &
        \frame{\includegraphics[height=\lenABSDFPlot]{imgs/validate_absdf_plot/palm_absdf_plot_setup.pdf}}
        &
        \frame{\includegraphics[height=\lenABSDFPlot]{imgs/validate_absdf_plot/palm_gt_+2ev.png}}
        &
        \frame{\includegraphics[height=\lenABSDFPlot]{imgs/validate_absdf_plot/palm_ours_2lobe_+2ev.png}}
        \\
        &
        (a) Setup & (b) Reference & (c) Ours
    \end{tabular}
    \caption{\label{fig:absdf_plot}
        Visualizing our factored ABSDF versus ground truth on two challenging cases. We select a voxel from each scene (a) and compare its reference ABSDF (b)
        to our factored ABSDF (c). Each plot contains $8 \times 8$ 2D outgoing slices in the lat-long coordinate system with different incident directions.
        Exposure is adjusted for clarity.}
\end{figure}

\subsection{Orientation-varying Parameters} \label{subsec:orient}
So far, we have assumed that $\beta^c$, $\beta^m$, and $\beta^s$ are independent of orientation in order to perform the split in Eq. \ref{eq:specular_orient_split} and
\ref{eq:diffuse_orient_split}, which prevents our method from supporting some important effects such as orientation-correlated color due to aggregation. In general,
one should stick to the joint distribution $p_{Y}(\gamma)$ to support arbitrary correlation. However, such high-dimensional distribution can be challenging to
represent and expensive to operate on. In our particular formulation, both the specular component and the diffuse component become a linear combination of
several spherical functions, each modulated by a linear combination of moments of $\beta^c$, $\beta^m$, and (or) $\beta^s$. We can extend our formulation by
making the moment terms directionally varying. Specifically, for the specular component, we would like to know the moments conditioned on a given half
vector direction $\omega_h$. The ``directional expectation'' can be defined as
\begin{equation} \label{eq:directional_moments}
    \mathbb{E}[\beta \,|\,\omega] = \frac{\int_A \beta_x D(R_x^T \omega;\alpha_x) \,\D{x}}{\int_A D(R_x^T \omega;\alpha_x) \,\D{x}},\\
\end{equation}
where $R_x$ is the tangent frame at $x$, and $D(R_x^T\omega;\alpha_x)$ is the microfacet distribution evaluated at the rotated $\omega$. The ``directional
second-order moments'' can be defined likewise. For the diffuse component, we replace the microfacet distribution with the SGs in Eq. \ref{eq:diffuse_sg}.

Now that the moment terms become directionally-varying, we can no longer store them as simple scalars. In practice, we find that it is usually sufficient to store
them in a very low resolution grid (e.g., $3\times3$) on the spherical domain because the angular frequency usually decreases as the scale of aggregation becomes 
larger. We demonstrate the neccessity of supporting orientation-varying parameters and the effectiveness of our method in 
Fig.~\ref{fig:orientation_varying_validation}.

\begin{figure}[t]
	\newlength{\heightsmall}
    \setlength{\heightsmall}{0.5in}
	\newlength{\heightbig}
    \setlength{\heightbig}{1.59in}
    \addtolength{\tabcolsep}{-4pt}
    \centering
    \begin{tabular}{ccccccc}
        \multicolumn{3}{c}{}
        &
        \includegraphics[height=\heightsmall]{imgs/redgreen/pt_redgreen.png}
        &
        \includegraphics[height=\heightsmall]{imgs/redgreen/ours_redgreen.png}
        &
        \includegraphics[height=\heightsmall]{imgs/redgreen/ablation_redgreen.png}
        &
        \raisebox{35pt}{\rotatebox{-90}{View 1}}
        \\
        \multicolumn{3}{c}{}
        &
        \includegraphics[height=\heightsmall]{imgs/redgreen/pt_red.png}
        &
        \includegraphics[height=\heightsmall]{imgs/redgreen/ours_red.png}
        &
        \includegraphics[height=\heightsmall]{imgs/redgreen/ablation_red.png}
        &
        \raisebox{35pt}{\rotatebox{-90}{View 2}}
        \\
        \multicolumn{3}{c}{\multirow[t]{3}{*}{\includegraphics[height=\heightbig]{imgs/redgreen/setup.png}}}
        &
        \includegraphics[height=\heightsmall]{imgs/redgreen/pt_green.png}
        &
        \includegraphics[height=\heightsmall]{imgs/redgreen/ours_green.png}
        &
        \includegraphics[height=\heightsmall]{imgs/redgreen/ablation_green.png}
        &
        \raisebox{35pt}{\rotatebox{-90}{View 3}}
        \\
        \multicolumn{3}{c}{(a) Setup} & (b) Ref. & (c) Ours & \tabincell{c}{(d) Na\"ive } &
    \end{tabular}
    \caption{\label{fig:orientation_varying_validation}
        Orientation-varying material parameters. (a) We aggregate a displaced surface with basecolor varying based on orientation and render it from 3 views.
        (b). Path-traced reference. The surface exhibits drastically different appearance from different views. (c). Our method correctly captures this
        view-dependent appearance. (d). Ignoring the orientation-vary parameters leads to incorrect results.}
\end{figure}

\subsection{Importance Sampling} \label{subsec:importance_sampling}
Our factored ABSDF allows straightforward importance sampling and PDF computation. This enables useful variance reduction techniques such as multiple importance
sampling (MIS). To sample the factored ABSDF $\hat{f}_\mathrm{novis}$:
\begin{enumerate}
    \item Pick one component between the specular and diffuse components. This can be done simply by uniform sampling.
    \item For the specular component, we first pick one convolved lobe from Eq. \ref{eq:sggx_conv_2} based on the lobe weights $w_j$. Then we sample the corresponding
          SGGX distribution.
    \item For the diffuse component, note that we cannot directly sample a convolved lobe from Eq. \ref{eq:diffuse_sg} because $\kappa_{ij}$ cannot be determined
          without $\omega_i$ (see Appendix). Therefore, we resort to a simple strategy by assuming a fixed $\kappa$ during importance sampling. The rest is
          similar to the specular case: we pick one convolved lobe (but with the fixed $\kappa$) and sample the corresponding SGGX distribution.
\end{enumerate}


==> old_rendering_theory.tex <==
\section{Far-field Scene Aggregation}
Our goal is to develop an appearance-preserving representation of a scene that is independent of the original geometry complexity, which we term \emph{scene
aggregate}. When measured externally, the general light transport of a scene aggregate can be characterized as an 8D function of incident/outgoing positions (on
a suitable manifold bound) and directions, similar to a BSSRDF. However, directly computing and storing such function is impractical due to the
prohibitive memory requirement. It is also not necessary as one might as well simply switch back to the original representation for near-field appearance.
Therefore, our formulation is based on the far-field assumption. When a scene is sufficiently far from the measuring sensor and
emitters that the sensor can no longer distinguish the internal spatial structure, we may drop the positional dependency by integrating the 8D light transport
function over positions. The resulting 4D function of incident/outgoing directions describes the far-field appearance of the scene aggregate and we name it
\emph{Aggregated Bidirectional Scattering Distribution Function} (ABSDF), again due to its similarity to a BSDF. Formally, we derive how to measure pixel
intensity from a scene aggregate with the definition of ABSDF.

\subsection{Defining ABSDF}
We consider a subset of a scene $A$ that consists of a set of surfaces. From a point $x \in A$, the outgoing radiance given some direct incident radiance
$L_i(x, \omega_i)$ is calculated by the rendering equation~\cite{kajiya86}:
\begin{align} \label{eq:rendering_eq}
\begin{split}
    &L_o(x, \omega_o) = \int_{\mathbb{S}^2} f(x, \omega_i, \omega_o) L_i(x, \omega_i) \langle n_x, \omega_i \rangle  V(x, \omega_i) \,\D{\omega_i}, \\
\end{split}
\end{align}
where $f(x, \omega_i, \omega_o)$ is the surface BSDF at $x$, and we explicitly write the visibility term $V(x, \omega_i)$.
We are interested in the average outgoing radiance from $A$ when viewed from  $\omega_o$, which can be written as a weighted average of per-point outgoing
radiance masked by another visibility term along $\omega_o$:
\begin{align} \label{eq:average_Lo}
\begin{split}
    L_o(\omega_o) &= \frac{1}{|A|_{\omega_o}} \int_{A}  L_o(x ,\omega_o) \langle n_x, \omega_o \rangle V(x, \omega_o) \,\D{x}, \\
    |A|_{\omega_o} &= \int_A \langle n_x\cdot\omega_o \rangle \,\D{x},
\end{split}
\end{align}
where $|A|_{\omega_o}$ is the projected area of $A$ along $\omega_o$. We can apply the far-field assumption such that the
incident radiance is independent of positions $L_i(x, \omega_i) \approx L_i(\omega_i)$ and rearrange Eq. \ref{eq:average_Lo}:
\begin{align} \label{eq:absdf_def}
\begin{split}
    L_o(\omega_o)
    &= \frac{1}{|A|_{\omega_o}} \int_{A} \Big( \int_{\mathbb{S}^2} f(x, \omega_i, \omega_o) \\
    &\quad L_i(\omega_i) \langle n_x, \omega_i \rangle  V(x, \omega_i) V(x, \omega_o) \,d\omega_i \Big)  \langle n_x, \omega_o \rangle \,\D{x} \\
    &= \int_{\mathbb{S}^2} \hat{f}(\omega_i, \omega_o) L(\omega_i) \,\D{\omega_i}, \\
    \hat{f}(\omega_i, \omega_o) &= \frac{1}{|A|_{\omega_o}} \int_A f(x,\omega_i, \omega_o) \langle n_x\cdot\omega_i \rangle \langle n_x\cdot\omega_o \rangle \\
    &\quad V(x,\omega_i)V(x,\omega_o)\,\D{x}. \\
\end{split}
\end{align}
We define $\hat{f}(\omega_i, \omega_o)$ as the ABSDF of $A$ as it captures the intrinsic geometrical and material characteristics of $A$ and is irrelevant to
external sensors or emitters. It is not hard to see that the ABSDF satisfies energy conservation as long as $f(x, \omega_i, \omega_o)$ is energy-conserving.
It also satisfies a generalized form of reciprocity that is similar to the situation in the microflake theory~\cite{jakob2010radiative}. To summarize:
\begin{align}
    &\int_{\mathbb{S}^2} \hat{f}(\omega_i, \omega_o) \,\D{\omega_i} \leq 1 \\
    &|A|_{\omega_o} \hat{f}(\omega_i, \omega_o) = |A|_{\omega_o} \hat{f}(\omega_o, \omega_i)
\end{align}

We note that it is possible to use the visible projected area\\
 $|A_v(\omega_o)| = \int_A \langle n_x \cdot \omega_o \rangle V(x, \omega_o) \,\D{x}$ as the normalization term in Eq.~\ref{eq:absdf_def}. In fact, the choice
 is not critical as the term will eventually be cancelled out (Eq.~\ref{eq:measure_eq_farfield},~\ref{eq:primitive_coverage}). We choose to use $|A|_{\omega_o}$
 for simplicity. In practice, neither $|A_v(\omega_o)|$  or $|A|_{\omega_o}$ needs to be computed or stored.

\subsection{Measuring Pixel Intensity} \label{subsec:measure_pixel}
Eq. \ref{eq:absdf_def} only defines the outgoing radiance, but ultimately our goal is to measure the pixel intensities contributed by the outgoing radiance
from $A$ arriving at the sensor.  Assuming a pinhole camera, the intensity of one pixel is defined as an additional integration over the film plane $\mathcal{F}$
\begin{align} \label{eq:measure_eq}
    I &= \int_{\mathcal{F}} W(x_\mathrm{f}) L_i(x_\mathrm{f}, \omega(x_\mathrm{f})) \,\D{x_\mathrm{f}},
\end{align}
where $x_f$ is a point on the film, $\omega(x_\mathrm{f})$ is corresponding ray direction originated from $x_\mathrm{f}$, $L_i(x_\mathrm{f}, \omega(x_\mathrm{f}))$
is the incident radiance on $x_\mathrm{f}$, and $W(x_\mathrm{f})$ is the reconstruction filter for this pixel.
\footnote{Strictly speaking, the pixel filter should be defined in the spatio-directional domain $\mathcal{F} \times \mathbb{S}^2$ that comprises all
directions through the pixel. Likewise, Eq. \ref{eq:measure_eq} should be an integration over $\mathcal{F} \times \mathbb{S}^2$. We avoid the technicality and
refer the readers to Veach~\shortcite{veach1998robust} for a more rigorous treatment.}
We assume the filter to be a box filter in this work for simplicity.
Let $P$ be the pixel footprint, the box filter is defined as $W(x) = 1 / |P|$ if $x \in P$ and 0 otherwise.

For $L_i(x_\mathrm{f}, \omega(x_\mathrm{f}))$, we first consider the scenario \emph{before} aggregation. The value of $L_i(x_\mathrm{f}, \omega(x_\mathrm{f}))$ depends
on whether the ray originated from $x_\mathrm{f}$ hits $A$:
\begin{enumerate}
    \item If the ray intersects $A$ one or more times, $L_i(x_\mathrm{f}, \omega(x_\mathrm{f}))$ evaluates to the outgoing radiance
            contributed by the first intersection point. However, we can also interpret it as the sum of the outgoing radiance
          contributed by each intersection point on $A$ masked by the outgoing visibility: \\
          $L_i(x_\mathrm{f}, \omega(x_\mathrm{f})) = \sum_k L_o(x_k, -\omega(x_\mathrm{f})) V(x_k, -\omega(x_\mathrm{f}))$.
    \item If the ray does not hit $A$, $L_i(x_\mathrm{f}, \omega(x_\mathrm{f}))$ evaluates to the radiance coming from the background:
          $L_i(x_\mathrm{f}, \omega(x_\mathrm{f})) = L_b(x_b, -\omega(x_\mathrm{f}))$, where $x_b$ refers to the hit point on the external boundary or infinity.
\end{enumerate}

Next, we consider the scenario \emph{after} aggregation. It is important to recall that the aggregated representation does not keep the original geometry.
Therefore, we can never perform ray tracing against $A$ during rendering. Instead, the scene will usually be discretized and $A$ will be replaced by a voxel
$\mathrm{v}$. We make the distinction that geometrically $A$ does not always have to be represented by the cubic shape of $\mathrm{v}$ itself. Instead, $A$ can be
represented by a different (simple) primitive $B$, the cubic shape being the simplest special case. In this work we reasonably assume $B$ defines a \emph{bounding volume}
of $A$. After aggregation, we only have knowledge of $B$.
We apply the far-field assumption such that the ray directions from points in the pixel footprint are constant $\omega(x_\mathrm{f}) \approx \omega_\mathrm{f}$.
Subsequently, the per-point outgoing radiance from $A$ is replaced with the average outgoing radiance $L_o(-\omega_\mathrm{f})$ (Eq. \ref{eq:average_Lo}) and
the background radiance depends on a fixed direction $L_b(x_b, -\omega(x_\mathrm{f})) \approx L_b(x_b, -\omega_\mathrm{f})$.
As illustrated in Fig.~\ref{fig:theory_illus1}, in this case, for a ray originated from $x_\mathrm{f}$:
\begin{enumerate}
    \item If the ray hits $B$, because $B$ is a bounding volume of $A$, it is possible for the ray to not hit $A$ and reach the background.
          Thus, we define the a binary function $C(x_\mathrm{f}, \omega_\mathrm{f})$ that detects whether the ray hits $A$ \emph{conditioned on it hitting $B$}.
          The value of $L_i(x_\mathrm{f}, \omega_\mathrm{f})$ is selected between $L_o(-\omega_\mathrm{f})$ and $L_b(x_b, -\omega_\mathrm{f})$ based on
          $C(x_\mathrm{f}, \omega_\mathrm{f})$.

    \item If the ray does not hit $B$, $L_i(x_\mathrm{f}, \omega_\mathrm{f})$ only includes the background radiance $L_b(x_b, -\omega_\mathrm{f})$.
\end{enumerate}

\begin{figure}[h]
	\newlength{\lenTheoryIllus}
	\setlength{\lenTheoryIllus}{1.5in}
	\centering
    \begin{overpic}[height=\lenTheoryIllus,unit=1mm]{imgs/illustration/theory_illustration_1.png}
        \put(5, 2){\normalsize $P$}
        \put(34, 2){\normalsize $\mathrm{v}$}
        \put(60, 35){\normalsize $\bm{A}$}
        \put(80, 12){\normalsize $B$}
    \end{overpic}
    \caption{\label{fig:theory_illus1} If a ray originated from the pixel footprint $P$ intersects $\mathrm{v}$, it may not intersect $B$ (green), intersect $B$ but not
            $A$ (yellow), or intersect $B$ and $A$ (red). The latter two cases are distinguished by the function $C(x_\mathrm{f}, \omega_{\mathrm{f}})$. }
\end{figure}

Therefore,
\begin{align} \label{eq:measure_eq_expand}
\begin{split}
    I = \frac{1}{|P|} \Big( &\int_{P^+} L_o(-\omega_\mathrm{f}) C(x_\mathrm{f}, \omega_\mathrm{f}) +
        L_b(x_b, -\omega_\mathrm{f}) (1 - C(x_\mathrm{f}, \omega_\mathrm{f})) \,\D{x_\mathrm{f}} \,+ \\
      &\int_{P^-} L_b(x_b, -\omega_\mathrm{f}) \,\D{x_\mathrm{f}} \Big),
\end{split}
\end{align}
where $P^+$ is the subset of $P$ including all points whose corresponding rays hit $B$ and $P^- = P \setminus P^+$. Note that the visibility terms are already
baked in $L_o(-\omega_\mathrm{f})$ (Eq.~\ref{eq:average_Lo}). This can be extended to handle multiple
disjoint subsets of the scene $\{A_k\}$, or in other words, accumulate the contributions from a list of voxels $\{\mathrm{v}_k\}$. We simply sum up
the contribution from each $A_k$:
\begin{align} \label{eq:measure_eq_expand_multi}
    \begin{split}
        I = \frac{1}{|P|} \Big(&\sum_k \int_{P^+_k} L_o^{A_k}(-\omega_\mathrm{f}) C_{A_k}(x_\mathrm{f}, \omega_\mathrm{f}) \,\D{x_\mathrm{f}} \,+ \\
          &\int_{P^+} L_b(x_b, -\omega_\mathrm{f}) V_b(x_\mathrm{f}, \omega_\mathrm{f}) \,\D{x_\mathrm{f}} \,+ \\
          &\int_{P^-} L_b(x_b, -\omega_\mathrm{f}) \,\D{x_\mathrm{f}} \Big),
    \end{split}
    \end{align}
where $P^+_k$ is the subset of $P$ including all points whose corresponding rays hit $B_k$, $P^+ = \bigcup_k P^+_k$, and $P^- = P \setminus P^+$.
For each $x_\mathrm{f}$, its associated ray may hit many $B_k$ but still reach the background as long as it does not hit any real geometry $A_k$.
Formally, we define another binary function $V_b(x_\mathrm{f}, \omega_\mathrm{f})$ that detects whether the ray is still unoccluded
\emph{conditioned on it hitting at least one $B_k$}.
We then apply the far-field assumption again such that the background radiance within the footprint is uncorrelated to the boundary visibility.
This simplifies Eq. \ref{eq:measure_eq_expand_multi} to
\begin{align} \label{eq:measure_eq_farfield}
\begin{split}
    I = &\sum_k \frac{|P^+_k|}{|P|} L_o^{A_k}(-\omega_\mathrm{f}) \hat{C}_{A_k}(\omega_\mathrm{f}) \,+ \\
        &\frac{|P^+|}{|P|} \hat{L}_b(-\omega_\mathrm{f})\hat{V_b}(\omega_\mathrm{f}) + \frac{|P^-|}{|P|} \hat{L}_b(-\omega_\mathrm{f}), \\
    &\hat{C}_{A_k}(\omega_\mathrm{f}; P^+_k) = \frac{1}{|P^+_k|} \int_{P^+_k} C_{A_k}(x_\mathrm{f}, \omega_\mathrm{f}) \,\D{x_\mathrm{f}}, \\
    &\hat{V}_b(\omega_\mathrm{f}; P^+) = \frac{1}{|P^+|} \int_{P^+} V_b(x_\mathrm{f}, \omega_\mathrm{f}) \,\D{x_\mathrm{f}}, \\
    &\hat{L}_b(-\omega_\mathrm{f}; P) = \frac{1}{|P|} \int_{P} L_b(x_\mathrm{f}, \omega_\mathrm{f}) \,\D{x_\mathrm{f}}, \\
\end{split}
\end{align}
where we define $|P_k^+|/|P|$ as the \emph{pixel coverage} of $\mathrm{v}_k$, $\hat{C}_{A_k}(\omega_\mathrm{f}; P^+_k)$ as the \emph{directional primitive coverage} of
$\mathrm{v}_k$, $\hat{V}_b(\omega_\mathrm{f}; P^+)$
as the \emph{aggregated boundary visibility} (ABV) of $A$, and $\hat{L}_b(-\omega_\mathrm{f}; P)$ as the average background radiance.
The definitions are illustrated in Fig.~\ref{fig:theory_illus2}.
The directional primitive coverage is local to each subset of the scene, while the ABV is global to the entire scene,
as it captures how the entire aggregate interacts with the external environment. Note that the ABV term only needs to be defined at the boundary of the entire
scene. Eq. \ref{eq:measure_eq_farfield} transfers to an efficient implementation because we can accumulate the contribution from each
$A_k$ in an order-independent manner.

\begin{figure}[h]
	\newlength{\lenTheoryIllusB}
	\setlength{\lenTheoryIllusB}{1.7in}
	\centering
    \begin{overpic}[height=\lenTheoryIllusB,unit=1mm]{imgs/illustration/theory_illustration_2.png}
        \put(1, 10){\normalsize $\hat{C}_{A_k}$}
        \put(1, 35){\normalsize $\frac{|P_k^+|}{|P|}$}
        \put(68, 2){\normalsize $\hat{V}_b$}
        \put(52, 8){\normalsize $\mathrm{v}_3$}
        \put(84, 8){\normalsize $\mathrm{v}_4$}
        \put(52, 41){\normalsize $\mathrm{v}_1$}
        \put(84, 41){\normalsize $\mathrm{v}_2$}
    \end{overpic}
    \caption{\label{fig:theory_illus2} Illustrating the pixel coverage of a voxel (top left), the directional primitive coverage a voxel (bottom left),
    and the aggregated boundary visibility of a scene that is subdivided into multiple voxels (right). }
\end{figure}

In summary, we have shown in theory how to define the aggregated representation of a given scene and how to render the aggregate. In the following sections,
we focus on two key aspects of our representation. In \S \ref{sec:factoring}, we detail our model
for ABSDF that captures the appearance of complex geometry and materials as well as its evaluation and importance sampling procedure. In \S \ref{sec:correlation},
we analyze how correlated geometry leads to challenges to compute coverage and visibility, and present our solution for them.

